Supervised Learning for Stochastic Optimal Control

Supervised machine learning is powerful. In recent years, it has enabled massive breakthroughs in computer vision and natural language processing. But leveraging these advances for optimal control has proved difficult. Data is a key limiting factor. Without access to the optimal policy, value function, or demonstrations, how can we fit a policy? In this paper, we show how to automatically generate supervised learning data for a class of continuous-time nonlinear stochastic optimal control problems. In particular, applying the Feynman-Kac theorem to a linear reparameterization of the Hamilton-Jacobi-Bellman PDE allows us to sample the value function by simulating a stochastic process. Hardware accelerators like GPUs could rapidly generate a large amount of this training data. With this data in hand, stochastic optimal control becomes supervised learning.

==> 07_discussion.tex <==
\section{Discussion}\label{sec:discussion}

\begin{itemize}
    \item Why it's good
    \begin{itemize}
        \item Offers a way to get training data for optimal control
        \item No expert policy needed. 
        \item Sample quality doesn't depend on previous learned values (as in RL, which can cause problems)
    \end{itemize}
    \item Some intuition: if just wiggling the control around a bit leads tVo low cost, this is probably a good state = good desirability. Even if you're far from the target, if just a few of the wiggles get you closer, then you get a good score. Make a plot of pendulum vector field, label a few points (e.g. (1), (2), (3)) and talk about them. At the desired operating point is obviously low cost. But close by and swinging the right direction is also good.
    \item Limitations
    \begin{itemize}
        \item Main thing is data hungryness: we can only sample $\Psi$ in expectation. Need several simulations for each $x^i$, and need $x^i$ sampled densely over the state space. Fortunately, GPU-based simulations put this in reach. 
        \item Tight interconnnection between noise, lambda, and R
        \item lambda (and therefore also noise and R) are important for conditioning: small lambda gives complementarity between desirability and value, too many zeros in training dataset is not that helpful. 
    \end{itemize}
    \item Future work
    \begin{itemize}
        \item Scale it up: this is an initial result. Still have a ways to go to catch up with RL. But, this is ready for scaling: can cheaply generate as much high-quality training data as you want
        \item Specialized architectures. CV has convolution. NLP has transformer. This has ??
        \item Use structure of PDE to regularize learning a la PINN. Large literature on PDE learning from fluids, etc to draw on. 
        \item Problem becomes badly conditioned as noise goes to zero. Noise-free optimal control extensions?
        \item Input limits and state constraints
        \item Quantum mechanics people have lots of tools for sampling from the FK PDE. Can we use them?
        \item The linearization doesn't work for noise-free systems. Can we extend to noise free by drawing connection between stochastic optimal controller and deterministic one? Emperically, the behavior is similar, and we just look at the limit as $\Sigma_\varepsilon \to 0$. But this also means $\lambda \to 0$, at which point $0 \leq V \bot \Psi \geq 0$.
    \end{itemize}
\end{itemize}

